Video Detective: Seek Critical Clues Recurrently to Answer Question from Long Videos

Long Video Question-Answering (LVQA) presents a significant challenge for Multi-modal Large Language Models (MLLMs) due to immense context and overloaded information, which could also lead to prohibitive memory consumption. While existing methods attempt to address these issues by reducing visual tokens or extending model's context length, they may miss useful information or take considerable computation. In fact, when answering given questions, only a small amount of crucial information is required. Therefore, we propose an efficient question-aware memory mechanism, enabling MLLMs to recurrently seek these critical clues. Our approach, named VideoDetective, simplifies this task by iteratively processing video sub-segments. For each sub-segment, a question-aware compression strategy is employed by introducing a few special memory tokens to achieve purposefully compression. This allows models to effectively seek critical clues while reducing visual tokens. Then, due to history context could have a significant impact, we recurrently aggregate and store these memory tokens to update history context, which would be reused for subsequent sub-segments. Furthermore, to more effectively measure model's long video understanding ability, we introduce GLVC (Grounding Long Video Clues), a long video question-answering dataset, which features grounding critical and concrete clues scattered throughout entire videos. Experimental results demonstrate our method enables MLLMs with limited context length of 32K to efficiently process 100K tokens (3600 frames, an hour-long video sampled at 1fps), requiring only 2 minutes and 37GB GPU memory usage. Evaluation results across multiple long video benchmarks illustrate our method can more effectively seek critical clues from massive information.

==> tabs/ablation_main.tex <==
% \begin{table*}[tbp]
% \belowrulesep=0pt
% \aboverulesep=0pt
% \begin{center}
% \caption{The main ablation results.}
% \vspace{-1em}
% \label{tab_main}
% % \abovetopsep=0pt
% % \aboverulesep=0pt
% % \belowrulesep=0pt
% % \belowbottomsep=0pt
% \scalebox{0.97}{
% \begin{tabular}{c|ccc|cc|c|c}
% % \hline
% % \bottomrule
% \toprule
% % \specialrule{1pt}{0pt}{0pt}
% & \multicolumn{3}{c|}{\textbf{Character}} & \multicolumn{2}{c|}{\textbf{Temporal}} &  &  \\
% \multirow{-2}{*}{\textbf{Method}} & \textbf{Action} & \textbf{Emotion} & \textbf{Motivation} & \textbf{Specific Time} & \textbf{Relationship} & \multirow{-2}{*}{\textbf{Plot}} & \multirow{-2}{*}{\textbf{Avg.}} \\
% \hline
% history information & 64.79 & 78.01 & 73.57 & 63.27 & 62.07 & 74.94 & 70.96  \\
% question-aware & 64.16 & 78.38 & 76.44 & 63.27 & 58.62 & 75.39 & 71.15 \\
% \hline
% \textbf{Ours} & 67.14 & 78.61 & 79.89 & 54.17 & 62.07 & 78.20 & 73.25 \\
% \bottomrule
% \end{tabular}
% }
% % \hdashline[0.5pt/3pt]
% \end{center}
% \vspace{-2em}
% \end{table*}





\begin{table}[tbp]
\belowrulesep=0pt
\aboverulesep=0pt
\begin{center}
\caption{Ablation results on history context and question-aware.}
\vspace{-1em}
\label{tab_ablation_main}
% \abovetopsep=0pt
% \aboverulesep=0pt
% \belowrulesep=0pt
% \belowbottomsep=0pt
\scalebox{0.65}{
\begin{tabular}{c|c|c|c|c}
% \hline
% \bottomrule
\toprule
% \specialrule{1pt}{0pt}{0pt}
\textbf{Method} & \textbf{Character-Avg} & \textbf{Temporal-Avg} &\textbf{Plot-Avg} & \textbf{Avg} \\
\hline
\emph{w/o.} history context & 69.96 & 62.82 & 74.94 & 70.96 \\
\emph{w/o.} question-aware & 70.16 & 61.54 & 75.39 & 71.15 \\
\hline
\textbf{Movie Detective (Ours)} & \textbf{74.13} & \textbf{75.64} & \textbf{80.54} & \textbf{75.91} \\
\bottomrule
\end{tabular}
}
% \hdashline[0.5pt/3pt]
\end{center}
\vspace{-2em}
\end{table}








==> tabs/tab_cinepile.tex <==
\begin{table}[tbp]
\belowrulesep=0pt
\aboverulesep=0pt
\begin{center}
\caption{The test results on Cinepile long video benchmark. The top 2 results for open-source and closed-source are highlighted.}
\vspace{-1em}
\label{tab_cinepile}
% \abovetopsep=0pt
% \aboverulesep=0pt
% \belowrulesep=0pt
% \belowbottomsep=0pt
\scalebox{0.65}{
\begin{tabular}{c|c|c|c|c|c|c|c}
% \hline
% \bottomrule
\toprule
% \specialrule{1pt}{0pt}{0pt}
\textbf{Model} & \textbf{Size} & \textbf{CRD} & \textbf{NPA} & \textbf{STA} & \textbf{TEMP} & \textbf{TH} & \textbf{Avg} \\
\hline
Gemini 1.5 Pro & - & \textbf{63.90} & \textbf{70.44} & \textbf{57.85} & \textbf{46.74} & \textbf{59.87} & \textbf{60.12} \\
Gemini 1.5 Flash & - & \underline{62.82} & \underline{69.76} & \underline{55.99} & \underline{44.04} & \underline{62.67} & \underline{58.75} \\
GPT-4o & - & 60.93 & 69.33 & 49.48 & 45.78 & 61.05 & 56.06 \\
GPT-4 Vision & - & 60.20 & 68.47 & 48.63 & 45.78 & 59.47 & 55.35 \\
\hline
LLaVA-OV~\cite{li2024llava} & 7B & 52.13 & \underline{59.83} & \underline{46.54} & 37.65 & \underline{58.42} & \underline{49.34} \\
LLaVA-OV Chat~\cite{li2024llava} & 7B & \underline{52.47} & 58.32 & 46.28 & \underline{37.79} & \underline{58.42} & 49.28 \\
MiniCPM-V 2.6~\cite{yao2024minicpm} & 8B & 50.10 & 54.21 & 44.52 & 35.61 & 54.74 & 46.91 \\
% Claude 3 Opus & - & 48.89 & 57.88 & 40.73 & 37.65 & 47.89 & 45.60 \\
VideoLLaMA 2~\cite{cheng2024videollama} & 7B & 47.44 & 54.64 & 41.91 & 34.30 & 47.37 & 44.57 \\
InternVL2~\cite{chen2024far} & 26B & 47.10 & 56.16 & 39.03 & 34.16 & 52.63 & 43.86 \\
% LongVA DPO & 7B & 45.84 & 54.21 & 39.16 & 33.43 & 44.74 & 42.78 \\
\hline
\textbf{Movie Detective (Ours)} & 7B & \textbf{56.43} & \textbf{63.47} & \textbf{57.23} & \textbf{40.31} & \textbf{64.15} & \textbf{55.36} \\
\bottomrule
\end{tabular}
}
% \hdashline[0.5pt/3pt]
\end{center}
\vspace{-2em}
\end{table}





==> tabs/tab_main.tex <==
\begin{table*}[tbp]
\belowrulesep=0pt
\aboverulesep=0pt
\begin{center}
\caption{The experiment results on M3QA test set. All models are fine-tuned on the M3QA training set except for video-SALMONN, which is used for inference with the official 13B model weights. The top2 results for open-source and closed-source are highlighted.
}
\vspace{-1em}
\label{tab_main}
% \abovetopsep=0pt
% \aboverulesep=0pt
% \belowrulesep=0pt
% \belowbottomsep=0pt
\scalebox{0.8}{
\begin{tabular}{c|c|ccc|cc|c|c}
% \hline
% \bottomrule
\toprule
% \specialrule{1pt}{0pt}{0pt}
&  & \multicolumn{3}{c|}{\textbf{Character}} & \multicolumn{2}{c|}{\textbf{Temporal}} &  &  \\
\multirow{-2}{*}{\textbf{Method}} & \multirow{-2}{*}{\textbf{Size}} & \textbf{Action} & \textbf{Emotion} & \textbf{Motivation} & \textbf{Specific Time} & \textbf{Relationship} & \multirow{-2}{*}{\textbf{Plot}} & \multirow{-2}{*}{\textbf{Avg}} \\
\hline
GPT-4o & - & \textbf{84.64} & \textbf{87.35} & \textbf{94.08} & \textbf{87.23} & \textbf{75.00} & \textbf{92.66} & \textbf{88.21} \\
% LLaMA 3.2 Vision  & & & & & & &  \\
\hline
video-SALMONN~\cite{sun2024video} & 13B & 33.86 & 26.73 & 45.76 & 36.73 & 36.67 & 40.04 & 35.50 \\
VideoLLaMA 2~\cite{cheng2024videollama} & 7B & 56.11 & 63.51 & 60.19 & 53.85 & 44.44 & 65.93 & 60.35 \\
Qwen2.5-VL~\cite{bai2025qwen2} & 7B & 63.41 & \underline{73.99} & 73.91 & \underline{63.41} & 54.19 & 68.41 & 67.84 \\
LLaMA-VID~\cite{li2024llama} & 7B & \underline{64.21} & 72.14 & \underline{80.34} & 59.32 & \underline{62.07} & \underline{71.34} & \underline{68.24} \\
\hline
\textbf{Movie Detective(Ours)} & 7B & \textbf{67.76} & \textbf{80.97} & \textbf{84.48} & \textbf{75.51} & \textbf{75.86} & \textbf{80.54} & \textbf{75.91} \\
\bottomrule
\end{tabular}
}
% \hdashline[0.5pt/3pt]
\end{center}
\vspace{-2em}
\end{table*}





==> tabs/tab_video_mme.tex <==
\begin{table}[tbp]
\belowrulesep=0pt
\aboverulesep=0pt
\begin{center}
\caption{The test results on Video-MME benchmark. The top2 results for open-source and closed-source are highlighted.}
\vspace{-1em}
\label{tab_video_mme}
% \abovetopsep=0pt
% \aboverulesep=0pt
% \belowrulesep=0pt
% \belowbottomsep=0pt
\scalebox{0.75}{
\begin{tabular}{c|c|c|c|c|c}
% \hline
% \bottomrule
\toprule
% \specialrule{1pt}{0pt}{0pt}
\textbf{Models} & \textbf{Size} & \textbf{Short} & \textbf{Medium} & \textbf{Long} & \textbf{Avg}  \\
\hline
Gemini 1.5 Pro & - & \textbf{81.7} & \textbf{74.3} & \textbf{67.4} & \textbf{75.0} \\
GPT-4V & - & \underline{70.5} & \underline{55.8} & \underline{53.5} & \underline{59.9} \\
\hline
Video-LLaVA~\cite{lin2023video} & 7B & 45.3 & 38.0 & 36.2 & 39.9 \\
ST-LLM~\cite{liu2024st} & 7B & 45.7 & 36.8 & 31.3 & 37.9 \\
VideoChat2-Mistral~\cite{li2024mvbench} & 7B & 48.3 & 37.0 & 33.2 & 39.5 \\
Chat-UniVi-V1.5~\cite{jin2024chat} & 7B & 45.7 & 40.3 & 35.8 & 40.6 \\
LLaVA-NeXT-Video~\cite{zhang2024llava} & 34B & \textbf{61.7} & \textbf{50.1} & \underline{44.3} & \textbf{52.0} \\
\hline
\textbf{Movie Detective(Ours)} & 7B & \underline{54.5} & \underline{49.9} & \textbf{45.8} & \underline{50.5} \\
\bottomrule
\end{tabular}
}
% \hdashline[0.5pt/3pt]
\end{center}
\vspace{-2em}
\end{table}




